Testing T2K's Bayesian constraints with priors in alternate parameterisations

Bayesian analysis results require a choice of prior distribution. In long-baseline neutrino oscillation physics, the usual parameterisation of the mixing matrix induces a prior that privileges certain neutrino mass and flavour state symmetries. Here we study the effect of privileging alternate symmetries on the results of the T2K experiment. We find that constraints on the level of CP violation (as given by the Jarlskog invariant) are robust under the choices of prior considered in the analysis. On the other hand, the degree of octant preference for the atmospheric angle depends on which symmetry has been privileged.

==> preamble.tex <==
\RequirePackage{fix-cm}
\RequirePackage{graphicx}
\RequirePackage[T1]{fontenc}

\smartqed  % flush right qed marks, e.g. at end of proof

\RequirePackage{amsfonts}
\RequirePackage{graphicx}
\RequirePackage{mathptmx} 
\RequirePackage{booktabs}
\RequirePackage{flushend}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

\RequirePackage{amsmath}
\RequirePackage{tikz}
\RequirePackage{xcolor}
\RequirePackage{cuted}
\RequirePackage{caption}

\setlength\stripsep{3pt plus 1pt minus 1pt}
%\usepackage{setspace}
%\usepackage{lineno}
%\usepackage{natbib}

%\linenumbers
%\renewcommand{\baselinestretch}{1.5}
